When Do Program-of-Thoughts Work for Reasoning?

In the realm of embodied artificial intelligence, the reasoning capabilities of Large Language Models (LLMs) play a pivotal role. Although there are effective methods like program-of-thought prompting for LLMs which uses programming language to tackle complex reasoning tasks, the specific impact of code data on the improvement of reasoning capabilities remains under-explored. To address this gap, we propose complexity-impacted reasoning score (CIRS), which combines structural and logical attributes, to measure the correlation between code and reasoning abilities. Specifically, we use the abstract syntax tree to encode the structural information and calculate logical complexity by considering the difficulty and the cyclomatic complexity. Through an empirical analysis, we find not all code data of complexity can be learned or understood by LLMs. Optimal level of complexity is critical to the improvement of reasoning abilities by program-aided prompting. Then we design an auto-synthesizing and stratifying algorithm, and apply it to instruction generation for mathematical reasoning and code data filtering for code generation tasks. Extensive results demonstrates the effectiveness of our proposed approach. Code will be integrated into the EasyInstruct framework at https://github.com/zjunlp/EasyInstruct.

==> commands.tex <==
\newcommand{\name}{ConCoRD}
\newcommand{\fullnameacronym}{Consistency Correction through Relation Detection}
\newcommand{\fullname}{Consistency correction through relation detection}
\newcommand{\fullnametitle}{Consistency Correction through Relation Detection}

\DeclareMathOperator*{\argmax}{argmax}


\definecolor{mygreen}{RGB}{50, 128, 50}
% \newcommand{\Sylvia}[1]{\textcolor{mygreen}{{\small \bf Siyan: #1}}}
\newcommand{\Sylvia}[1]{}
\newcommand{\quotestring}[1]{\textit{#1}}

% Chris's comments. At the end you can turn this off either by changing the below line to \commentsfalse or deleting all \cm.* commands and this block.
\newif\ifcomments
\commentstrue
\ifcomments
\usepackage[normalem]{ulem}
\definecolor{CMpurple}{rgb}{0.6,0.18,0.64}
\newcommand\cm[1]{\textcolor{CMpurple}{\textsf{\scriptsize[\textbf{CM\@:} #1]}}}
\newcommand\cmi[1]{\textcolor{CMpurple}{#1}}
\newcommand\cmm[1]{\marginpar{\raggedright\tiny\textcolor{CMpurple}{\textsf{{\bfseries CM\@:} #1}}}}
\newcommand\cms{\bgroup\markoverwith{\textcolor{CMpurple}{\rule[.4ex]{2pt}{0.8pt}}}\ULon}
\else
\newcommand\cm[1]{}
\newcommand\cmi[1]{\ignorespaces}
\newcommand\cmm[1]{}
\newcommand\cms[1]{#1}
\fi




==> tables/experiment-ablation-code.tex <==
\begin{table*}[h]
\centering
% \scalebox{1.0}{
\begin{tabular}{llllllllll}
\toprule
 & & \multicolumn{8}{c}{CoT Reasoning on Maths   Word Problems} \\ \cline{3-10} 
 &  & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{MultiArith} & \multicolumn{2}{c}{ASDiv} & \multicolumn{2}{c}{SVAMP} \\ \cline{3-10} 
Models             & \#Params        & Acc.    &     & Acc.    &     & Acc.    &    & Acc.   &    \\

\midrule
Llama &   7B &     & &     & &    &        &    \\
Llama-LOW &   7B &     & &     & &    &        &    \\
Llama-MEDIUM &   7B &     & &     & &    &        &    \\
Llama-HIGH &  7B   &     & &     & &    &        &    \\
\midrule
Llama &  13B &     & &     & &    &        &    \\
Llama-LOW & 13B &     & &     & &    &        &    \\
Llama-MEDIUM & 13B &     & &     & &    &        &    \\
Llam-HIGH  & 13B &     & &     & &    &        &    \\
\midrule
Llama &  30B &     & &     & &    &        &    \\
Llama-LOW & 30B &     & &     & &    &        &    \\
Llama-MEDIUM & 30B &     & &     & &    &        &    \\
Llam-HIGH  & 30B &     & &     & &    &        &    \\
\midrule
Llama &  65B &     & &     & &    &        &    \\
Llama-LOW & 65B &     & &     & &    &        &    \\
Llama-MEDIUM & 65B &     & &     & &    &        &    \\
Llam-HIGH  & 65B &     & &     & &    &        &    \\
\bottomrule
\end{tabular}
% }
\caption{Ablation-Pure code impacts.
}
\end{table*}



==> tables/experiment-example-score.tex <==
% \begin{table*}[h]
% \small
% \centering
% \begin{tabularx}{\linewidth}{lX}
% \toprule
% \textbf{\textit{Human:}} &
%   How to save data into a json file in Python? \\
%   \midrule
%   \textbf{\textit{Baize-7B:}} & One way to do this in Python is to use the json module and write the json data to a file using the built-in \texttt{json.dump()} method. Here's an example:
  
%   \usebox\codea

%   You can use the \texttt{json\_file} variable to specify the file path where you want to save the json data. The \texttt{json.dump()} method will write the json data to the specified file path.
% \\
% \midrule
% \textbf{\textit{Human:}} & Rewrite the code as a function. Data and file path as parameters. \\
%   \midrule
% \textbf{\textit{Baize-7B:}} & 
% Here's the rewritten code:

% \usebox\codeb

% The function \texttt{save\_json()} will call the \texttt{json.dump()} method on the given \texttt{data} object, passing it as the first argument and the file path as the second argument. The function \texttt{save\_json()} will also open a file with the specified file path and call the \texttt{json.dump()} method on that object. \\

 
% \bottomrule  
% \end{tabularx}
% \caption{\textit{(Cherry-picked)} An example of interactive coding via dialogue. \label{tab:code_dialog_example}}
% \end{table*}

\begin{table*}[h]
\small
\centering
\begin{tabularx}{\linewidth}{lX}
\toprule

\textbf{\textit{low score}} &
\textbf{Input:}
How many of the positive factors of 24 are not factors of 60?
\textbf{Output:}
```python
\# The factors of 24 are: 1, 2, 3, 4, 6, 8, 12, 24
\# The factors of 60 are: 1, 2, 3, 4, 5, 6, 10, 12, 15, 20, 30, 60
\# To find the factors of 24 that are not factors of 60, we can subtract the factors of 60 from the factors of 24
\# The factors of 24 that are not factors of 60 are: 8, 24
\# Therefore, there are 2 factors of 24 that are not factors of 60
``` 
\\

\midrule

\textbf{\textit{medium score}} & 
\textbf{Input:} A store is having a sale on shirts. if you buy 3 shirts, you get 20\% off the total price. if a shirt costs \$25, how much would it cost to buy 3 shirts during the sale
\textbf{Output:} ```python shirt\_price $=$ 25 num\_shirts $=$ 3 total\_price $=$ shirt\_price $*$ num\_shirts discounted\_price $=$ total\_price $*$ 0.8 print(discounted\_price)```
\\

\midrule
\textbf{\textit{high score}} &
\textbf{Input:}
A group of five students have tickets for six adjacent seats in one row of a classroom. If two of the students refuse to sit next to each other, how many possible different seating arrangements are there for these 6 students?
\textbf{Output:}
```python
from itertools import permutations
students = ['A', 'B', 'C', 'D', 'E', 'F']
seats = ['S1', 'S2', 'S3', 'S4', 'S5', 'S6']
count = 0
for arrangement in permutations(students, len(students)):
    if 'A' in arrangement and 'B' in arrangement:        if arrangement.index('A') $==$ arrangement.index('B') $+$ 1 or arrangement.index('A') $==$ arrangement.index('B') $-$ 1:
            continue
...
```
\\
 
\bottomrule  
\end{tabularx}
\caption{Examples of different complexity score distributions. \label{table:example-score}}
\end{table*}

==> tables/experiment-overall.tex <==
\begin{table*}[h]
\centering
% \scalebox{1.0}{
\begin{tabular}{llllllllll}
\toprule
 & & \multicolumn{8}{c}{CoT Reasoning on Maths   Word Problems} \\ \cline{3-10} 
 &  & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{MultiArith} & \multicolumn{2}{c}{ASDiv} & \multicolumn{2}{c}{SVAMP} \\ \cline{3-10} 
Models             & \#Params        & Acc.    &  -   & Acc.    &  -   & Acc.    &  -  & Acc.   &  -  \\
\midrule
code-davinci-002 & $\ge$ 175B & 11.20  & - &  11.40  & - & 48.30 & - &  53.80 & - \\
text-davinci-003 & $\ge$ 175B & 11.87   & - &  11.80  & - & 48.90 &  -&  61.60  & -\\
GPT-3.5-turbo & $\ge$ 175B & 65.18   & - &  84.80  & - & 74.39 & - &  71.00  & -\\

\midrule
Llama &   7B &  final testing remained   & - &    & - &  & - &   & -  \\
% Llama-textual rationale &   7B &   data-generating   & - &    & - &   & - & & -  \\
% Llama-code instruction &   7B &    data-generating    & - &     & - &  & - & & -  \\
Llama-random code &   7B &    & - &     & - &   & - &    & -  \\
Llama-LOW &   7B & under inference   & - &     & - &   & - &    & -  \\
Llama-MEDIUM &   7B &  under inference     & - &     & - &   & - &    & -  \\
Llama-HIGH &  7B  &   under inference    & - &     & - &   & - &    & -  \\

\midrule
Llama &  13B  & final testing remained    & - &    & - &  & - &   & -  \\
% Llama-textual rationale  &   13B & data-generating    & &     & &    &        &    \\
% Llama-code instruction &   13B &  data-generating   & &     & &    &        &    \\
Llama-random code & 13B  &       & - &     & - &   & - &    & -  \\
Llama-LOW & 13B  &  under inference     & - &     & - &   & - &    & -  \\
Llama-MEDIUM & 13B  &       & - &     & - &   & - &    & -  \\
Llam-HIGH  & 13B  &      & - &     & - &   & - &    & -  \\
% \midrule
% Llama &  30B &     & &     & &    &        &    \\
% Llama-textual rationale  &   30B &     & &     & &    &        &    \\
% Llama-code instruction &   30B &     & &     & &    &        &    \\
% Llama-LOW & 30B &     & &     & &    &        &    \\
% Llama-MEDIUM & 30B &     & &     & &    &        &    \\
% Llam-HIGH  & 30B &     & &     & &    &        &    \\
% \midrule
% Llama &  65B &     & &     & &    &        &    \\
% Llama-textual rationale  &   65B &     & &     & &    &        &    \\
% Llama-code instruction &   65B &     & &     & &    &        &    \\
% Llama-LOW & 65B &     & &     & &    &        &    \\
% Llama-MEDIUM & 65B &     & &     & &    &        &    \\
% Llam-HIGH  & 65B &     & &     & &    &        &    \\
\bottomrule
\end{tabular}
% }
\caption{Overall test set performance.}
\end{table*}


% \newcommand{\sepsmall}[0]{\hspace{4pt}}
% \newcommand{\septiny}[0]{\hspace{8pt}}
% \begin{table*}[th!]
%   \caption{
%   Overall test set performance. We specialize Flan-T5's ability from the generic tasks (BigBench Hard) to math reasoning tasks.
%   After paying the cost of BigBench Hard performance (the model loses all the CoT prompting ability and a large portion of the Answer-only (AO) prompting ability), we see the specialized T5 models have improved in-distribution (GSM8K) performance (where our 3B and 11B models outperform concurrent works) as well as out-of-distribution (MultiArith, ASDiv and SVAMP) performance, showing that we can move the model's ability from generic tasks (BBH) to a specific target task (math reasoning). 
%   % Magister22: \citet{magister2022teaching};
%   % Shridhar22: \citet{shridhar2022distilling};
%   % Ho22: \citet{ho2022large}.
%   }
%   \label{tab:exp:overall}
%   \centering
%   \setlength{\tabcolsep}{4pt}

% \begin{tabular}{@{}l@{}r@{\hskip 16pt}|c@{\sepsmall}c|m{0.01em}|c@{\sepsmall}c|m{0.01em}|c@{\sepsmall}c|m{0.01em}|c@{\sepsmall}c|m{0.01em}|@{\hskip 8pt}|c@{\sepsmall}c|m{0.01em}|c@{\sepsmall}c|@{}}

%       \toprule[1.25pt]
      
%        &&  \multicolumn{11}{c}{\textbf{CoT Reasoning on Maths Word Problems}} && \multicolumn{5}{c}{\textbf{BigBench-Hard}} \\ 
%        \cmidrule(lr){3-13}
%        \cmidrule(lr){15-19}
%         & & \multicolumn{2}{c}{\textbf{GSM8K}} && \multicolumn{2}{c}{\textbf{MultiArith}} && \multicolumn{2}{c}{\textbf{ASDiv}} && \multicolumn{2}{c}{\textbf{SVAMP}} 
%         && \multicolumn{2}{c}{\textbf{AO}} && \multicolumn{2}{c}{\textbf{CoT}} \\
%        \cmidrule(lr){3-4}
%        \cmidrule(lr){6-7}
%        \cmidrule(lr){9-10}
%        \cmidrule(lr){12-13}
%        \cmidrule(lr){15-16}
%        \cmidrule(lr){18-19}
%         \textbf{Models}
%         & \textbf{\#Params.} 
%         &   \textbf{Acc.} & $\mathbf{\Delta}$
%         &&  \textbf{Acc.} & $\mathbf{\Delta}$
%         &&  \textbf{Acc.} & $\mathbf{\Delta}$
%         &&  \textbf{Acc.} & $\mathbf{\Delta}$
%         &&  \textbf{Acc.} & $\mathbf{\Delta}$
%         &&  \textbf{Acc.} & $\mathbf{\Delta}$\\
        
%       \midrule[1.25pt]
        
%         %%%
%         code-davinci-002 & $\ge$175B 
%         &  63.1 & - 
%         && 95.8 & - 
%         && 80.4 & - 
%         && 76.4 & - 
%         && 56.6 & - 
%         && 73.9 & -\\ 
%         %%%

%         %%%
%         LaMDA & 137B 
%         &  14.8 & - 
%         && 45.0 & - 
%         && 46.6 & - 
%         && 37.5 & - 
%         && -    & - 
%         && -    & -  \\ 
%         %%%

%         %%%
%         PaLM & 60B 
%         &  29.9 & - 
%         && 75.0 & - 
%         && 61.9 & - 
%         && 46.7 & - 
%         && 37.4 & - 
%         && 43.0 & - \\ 
%         %%%

%         %%%
%         UL2 & 20B 
%         & {0}4.4 & - 
%         && -    & - 
%         && 16.9 & - 
%         && 12.5 & - 
%         && -    & - 
%         && -    & - \\ 
%         %%%

%       \midrule[1.25pt]
%         \multicolumn{18}{@{}l}{\textbf{Concurrent Works with Knowledge Distillation}}\\
%       Magister22, T5
%       % \citet{magister2022teaching} T5 
%       & 11B 
%       &  21.9  & - 
%       && -    & - 
%       && 42.1 & - 
%       && -    & - 
%       && ?    & - 
%       && ?    & - \\
      
      
%       Shridhar22, GPT
%       %\citet{shridhar2022distilling}  GPT 
%       & 6B 
%       & 21.0 & -  
%       && -   & -  
%       && -   & - 
%       && -   & - 
%       && ?   & - 
%       && ?   & - \\


      
%       Ho22, GPT
%       % \citet{ho2022large}  
%       & 6B 
%       & {0}6.8 & - 
%       && 33.3 & - 
%       && -    & - 
%       && -    & - 
%       && ?    & - 
%       && ?    & - \\ 

%       \midrule[1.25pt]
%       \multicolumn{18}{@{}l}{\textbf{Our Specialized Models Compared with Baselines}}\\
      
%       FlanT5-XXL 
%       & 11B 
%       &  16.1 & - 
%       && 51.7 & - 
%       && 36.5 & - 
%       && 39.7 & - 
%       && 47.4 & - 
%       && 41.8 & - \\ 
      
      
%       \; + Specialized 
%       &  11B  
%       &  27.1  & {+11.0} 
%       && 63.0 & {+11.3} 
%       && 37.6 & {0}{+1.1} 
%       && 35.6 & {0}{-4.1} 
%       && 19.6 & {-27.8} 
%       && {0}0.0  & {-41.8} \\ 
      
      
      
    
%       \midrule[0.5pt]
      
      
      
%       FlanT5-XL 
%       & 3B 
%       &  13.5 & -
%       && 24.0   & -  
%       && 20.7 & - 
%       && 17.7 & - 
%       && 39.9 & - 
%       && 35.8 & - \\ 
%       \; + Specialized 
%       & 3B  
%       &  22.4 & {0}{+8.9} 
%       && 42.3 & {+18.3} 
%       && 28.4 & {0}{+7.7} 
%       && 23.8 & {0}{+6.1} 
%       && {0}3.2  & {-36.7} 
%       && {0}0.0  & {-35.8} \\ 
      
%       \midrule[0.5pt]
      
%       FlanT5-Large 
%       & 760M 
%       &  {0}6.9  & - 
%       && 13.0 & - 
%       && 10.1 & - 
%       && {0}6.8  & - 
%       && 30.3 & - 
%       && 30.9 & - \\ 
      
      
%       \; + Specialized 
%       & 760M  
%       &  20.2 & {+13.3} 
%       && 38.5 & {+25.5} 
%       && 23.8 & {+13.7} 
%       && 20.4 & {+13.6} 
%       && {0}6.5  & {-23.8} 
%       && {0}0.3 & {-30.6} \\ 
      
%       \midrule[0.5pt]
      
%       FlanT5-Base 
%       & 250M 
%       &  {0}3.0  & - 
%       && {0}7.0  & - 
%       && {0}4.2  & - 
%       && {0}3.8  & - 
%       && 24.2 & - 
%       && 25.9 & - \\ 
      
%       \; + Specialized
%       & 250M  
%       &  13.4 & {+10.4} 
%       && 29.7 & {+22.7} 
%       && 20.9 & {+16.7} 
%       && 14.2 & {+10.4} 
%       && {0}3.1  & {-21.1} 
%       && {0}0.1 & {-25.8}\\ 
      
%       \bottomrule[1.25pt]
%   \end{tabular}
% \end{table*}



==> tables/experiment-template.tex <==
% \begin{table*}[h]
% \small
% \centering
% \begin{tabularx}{\linewidth}{lX}
% \toprule
% \textbf{\textit{Human:}} &
%   How to save data into a json file in Python? \\
%   \midrule
%   \textbf{\textit{Baize-7B:}} & One way to do this in Python is to use the json module and write the json data to a file using the built-in \texttt{json.dump()} method. Here's an example:

  
%   \usebox\codea

%   You can use the \texttt{json\_file} variable to specify the file path where you want to save the json data. The \texttt{json.dump()} method will write the json data to the specified file path.
% \\
% \midrule
% \textbf{\textit{Human:}} & Rewrite the code as a function. Data and file path as parameters. \\
%   \midrule
% \textbf{\textit{Baize-7B:}} & 
% Here's the rewritten code:

% \usebox\codeb

% The function \texttt{save\_json()} will call the \texttt{json.dump()} method on the given \texttt{data} object, passing it as the first argument and the file path as the second argument. The function \texttt{save\_json()} will also open a file with the specified file path and call the \texttt{json.dump()} method on that object. \\

 
% \bottomrule  
% \end{tabularx}
% \caption{\textit{(Cherry-picked)} An example of interactive coding via dialogue. \label{tab:code_dialog_example}}
% \end{table*}

\begin{table*}[h]
\small
\centering
\begin{tabularx}{\linewidth}{lX}
\toprule
% Problem: There are 24 students in the class. One-third had their school portraits taken before lunch. After lunch, but before gym class, 10 additional students had their portraits taken. After gym class, how many students have not yet had their picture taken?
% Problem: An old pirate wants to leave his treasure on an island. He has 3500 gold coins. He wants to spread this equally across 5 chests. Additionally, he will put a total of 500 silver coins and twice as many bronze coins as silver, all distributed equally across the chests. How many coins in total will be in each chest?
% Problem: Maria wants to paint a picture and needs some tools to do that. She wants to buy a set of brushes for $20 and some canvas for three times more than the brushes. The paint costs Maria $8 per liter, and she needs at least 5 liters. How much money will she earn on the painting if she will be able to sell it for $200?

\textbf{\textit{Instruction:}} &
  Below are some mathematical problems. Can you rewrite new problems that are similar to them? Then you should write python code to sovle the new problem. Note that when you write codes, please wrap them with ```.  \\

\midrule

\textbf{\textit{Input:}} &
    \textbf{Problem:} There are 24 students in the class. One-third had their school portraits taken before lunch. After lunch, but before gym class, 10 additional students had their portraits taken. After gym class, how many students have not yet had their picture taken?
    
    \textbf{Problem:}  An old pirate wants to leave his treasure on an island. He has 3500 gold coins. He wants to spread this equally across 5 chests. Additionally, he will put a total of 500 silver coins and twice as many bronze coins as silver, all distributed equally across the chests. How many coins in total will be in each chest?
    
    \textbf{Problem:} Maria wants to paint a picture and needs some tools to do that. She wants to buy a set of brushes for \$20 and some canvas for three times more than the brushes. The paint costs Maria \$8 per liter, and she needs at least 5 liters. How much money will she earn on the painting if she will be able to sell it for \$200?. \\

\midrule

\textbf{\textit{Output:}} & \textbf{New problem 1:} There are 30 students in the class. Two-fifths had their school portraits taken before lunch. After lunch, but before gym class, 15 additional students had their portraits taken. After gym class, how many students have not yet had their picture taken?
\textit{```python
total\_students $=$ 30
portraits\_before\_lunch $=$ total\_students $*$ 2 $/$ 5
portraits\_after\_lunch $=$  portraits\_before\_lunch $+$ 15
students\_without\_portraits $=$  total\_students $-$ portraits\_after\_lunch
print(students\_without\_portraits)
```}

...
\\
 
\bottomrule  
\end{tabularx}
\caption{An example of data generator instruction and templates. }
\label{table:template}
\end{table*}
